Solving Marginal MAP Problems with NP Oracles and Parity Constraints

Arising from many applications at the intersection of decision making and machine learning, Marginal Maximum A Posteriori (Marginal MAP) Problems unify the two main classes of inference, namely maximization (optimization) and marginal inference (counting), and are believed to have higher complexity than both of them. We propose XOR_MMAP, a novel approach to solve the Marginal MAP Problem, which represents the intractable counting subproblem with queries to NP oracles, subject to additional parity constraints. XOR_MMAP provides a constant factor approximation to the Marginal MAP Problem, by encoding it as a single optimization in polynomial size of the original problem. We evaluate our approach in several machine learning and decision making applications, and show that our approach outperforms several state-of-the-art Marginal MAP solvers.

==> Makefile <==
.PHONY: main fromscratch dvi ps pdf bibs xfigs compact clean tar tgz

TEXFILE    = decision_making_counting

LATEX      = latex
BIBTEX     = bibtex
MAKEINDEX  = makeindex
DVIPS      = dvips -t letter
PDFLATEX   = pdflatex
PS2PDF     = ps2pdf
XFIGDIR     = xfigs
CURRENTDIR = `basename "\`pwd\`"`

default: pdf

#fromscratch: xfigs
fromscratch:
	$(LATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

dvi:
	$(LATEX) $(TEXFILE)

ps: dvi
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

pdf:
	# $(LATEX) $(TEXFILE)
	# $(BIBTEX) $(TEXFILE)
	# $(LATEX) $(TEXFILE)
	# $(LATEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
#pdf: ps
#$(PS2PDF) $(TEXFILE)

bibs:
	$(BIBTEX) $(TEXFILE)

xfigs:
	(cd $(FIGDIR); bash ./makefigs ../*.tex )

compact:
#	(rm -f *.aux *.log *.blg *.out *.toc $(TEXFILE).bbl)
	(rm -f *.aux *.log *.blg *.out *.toc)

clean: compact
#	(rm -f *.dvi *.ps *.pdf $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )
	(rm -f *.dvi *.ps *.pdf $(TEXFILE).bbl $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )

tar:
	rm -f ../$(CURRENTDIR).tar.gz
	tar cvf ../$(CURRENTDIR).tar ../$(CURRENTDIR)
	gzip ../$(CURRENTDIR).tar
	echo "Created ../$(CURRENTDIR).tar.gz"

tgz:
	rm -f ../$(CURRENTDIR).tgz
	tar cvfz ../$(CURRENTDIR).tgz ../$(CURRENTDIR)
	echo "Created ../$(CURRENTDIR).tgz"



==> README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

